RUCA: RUntime Configurable Approximate Circuits with Self-Correcting Capability

Approximate computing is an emerging computing paradigm that offers improved power consumption by relaxing the requirement for full accuracy. Since real-world applications may have different requirements for design accuracy, one trend of approximate computing is to design runtime quality-configurable circuits, which are able to operate under different accuracy modes with different power consumption. In this paper, we present a novel framework RUCA which aims to approximate an arbitrary input circuit in a runtime configurable fashion. By factorizing and decomposing the truth table, our approach aims to approximate and separate the input circuit into multiple configuration blocks which support different accuracy levels, including a corrector circuit to restore full accuracy. By activating different blocks, the approximate circuit is able to operate at different accuracy-power configurations. To improve the scalability of our algorithm, we also provide a design space exploration scheme with circuit partitioning to navigate the search space of possible approximations of subcircuits during design time. We thoroughly evaluate our methodology on a set of benchmarks and compare against another quality-configurable approach, showcasing the benefits and flexibility of RUCA. For 3-level designs, RUCA saves power consumption by 36.57% within 1% error and by 51.32% within 2% error on average.

==> old_meth.tex <==
Line 1-19 of Algorithm~\ref{alg:rc} describes our methodology. An input circuit with $n$ inputs and $m$ outputs is first simulated into truth table $\textbf{M}$ of size $2^n \times m$ (line 1). Our objective is to generate a runtime configurable approximate circuit which implements a list of objective errors $\epsilon=[\epsilon_1, \epsilon_2, \cdots]$ in descending order (line 2). Boolean matrix $\textbf{M}$ is factorized into $\textbf{B}_f$ and $\textbf{C}_f$ with factorization degree $f$ ranging from $1$ to $m-1$ (line 6), where error $|\textbf{M} - \textbf{B}_f\textbf{C}_f|$
is assessed for each factorization degree respectively (line 7). As $f$ increases, error becomes smaller. We start by searching for the smallest factorization degree $f_1$ that meets the requirement of largest objective error such that $|\textbf{M} - \textbf{B}_{f_1}\textbf{C}_{f_1}| \leq \epsilon_1$ (line 8). The first $f_1$ columns of $\textbf{B}$ and first $f_1$ rows of $\textbf{C}$ are then synthesized into circuits, which are combined into circuit $Cir_1$ as the first accuracy level of approximate circuit (line 9-12). Next, the factorization degree $f_2$ is searched to meet the second smallest objective error such that $|\textbf{M} - \textbf{B}_{f_2}\textbf{C}_{f_2}| \leq \epsilon_2$. The $(f_1+1)^{th}$ to $f_2^{th}$ pairs of columns and rows are synthesized as the second section $Cir_2$ of approximate circuit. With semi-ring algebra ($1+1=1$) in BMF algorithm, two sections $Cir_1$ and $Cir_2$ are connected with logic OR for corresponding outputs. In order to reach error threshold $\epsilon_2$, we keep both sections $Cir_1$ and $Cir_2$ active. However, if a specific application only requires error threshold $\epsilon_1$, we can then shut down $Cir_2$ and only keep $Cir_1$ running. Previous work is repeated until we find such factorization degree for each objective error (line 16-18). As discussed above, to implement error threshold $\epsilon_i$, we may keep first $i$ sections running and shut down the rest. Thus, we split factorized truth table into groups of column-row pair and synthesize each group into sections separately. Each section is expected to have a much lower power consumption than original circuit. By shutting down different number of sections at runtime, approximate circuit is able to dynamically control the trade-off between design accuracy and power consumption. 

Figure~\ref{fig:general_flow} demonstrates an example, where we factorize input truth table into two groups of columns and rows. The first group has two pairs of columns and rows, which is then synthesized into section 1 ($C1$ and $D1$). The second group has one pair, which is synthesized into section 2 ($C2$ and $D2$). Two sections are connected with bitwise OR gate (gate $a$). In the case that the application can tolerate relatively large error, we only keep $C1$ and $D1$ running. If we need more accurate results, we further turn on $C2$ and $D2$ to optimize Quality of Results (QoR). But the power consumption will increase due to this additional running section.

\begin{algorithm}[t!]
	\footnotesize
	\SetKwBlock{Begin}{begin}{end}
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	%\SetKwInOut{Phase1}{Phase 1}
	\Input{Accurate Circuit $ACir$ with $n$ inputs and $m$ outputs, List of Objective Errors $\epsilon$}\label{alg:input}
	\Output{List of Approximate Sections $\textbf{Cir}$, Corrector Circuit $Cir_c$}
	$\textbf{M}$ = Simulate accurate circuit $ACir$\\
	Sort list of objective errors $\epsilon$ in descending order \\
	$\textbf{Cir}$ = empty list \\
	$prev\_f$ = 0  // Denote factorization degree for previous section \\
	\For{factorization degree f in 1 to m-1 }
    {
        [$\textbf{B}_f$, $\textbf{C}_f$] = BMF($\textbf{M}$, f) \\
        err = $|\textbf{M} - \textbf{B}_f\textbf{C}_f|$ \\
        \If{err \leq $\epsilon[0]$}
        {
        $Cir_B$ = Synthesize columns in range $(prev\_f, f]$ of $\textbf{B}_f$ \\
        $Cir_C$ = Synthesize rows in range $(prev\_f, f]$ of $\textbf{C}_f$ \\
        $Cir'$ = Connect $Cir_B$ $Cir_C$ and optimize \\
        $\textbf{Cir}$.append($Cir'$) \\
        $prev\_f$ = $f$ \\
        $\epsilon$.pop(0)\\
        }
        \If{$\epsilon$ is empty} {break \\}
    
    }	
	$\textbf{R}$ = bitwise\_XOR($\textbf{M}$, $\textbf{B}_f\textbf{C}_f$) \\
	$Cir_c$ = Synthesize corrector matrix $\textbf{R}$ \\
	\Return $\textbf{Cir}$, $Cir_c$
	\caption{Runtime Configurable Approximate Circuit with Self Correcting Capability}
		\label{alg:rc}
	%\vspace{-0.1in}
\end{algorithm}


\subsection{Self Correcting Capability}
\label{sec:capability}
In previous subsection, we discuss the methodology of generating runtime configurable approximate circuits with Boolean matrix factorization. Since BMF is NP-hard, in most cases, we are not able to reconstruct input matrix accurately. In order to also support applications which require 100\% accuracy, we propose a corrector circuit to implement self correcting capability. 

Suppose we have a list of factorization degrees $[f_1, f_2, \cdots]$ corresponding to various accuracy level, where $f_n$ is the factorization degree for smallest objective error. Truth table of approximate circuits in degree $f_n$ is $\textbf{M}_{f_n}=\textbf{B}_{f_n}\textbf{C}_{f_n}$. To restore flipped bits in truth table, field modulo-2 algebra is used, where `1's can be used to flip bits such as $1+1=0$ and $1+0=1$. As line 20-21 of Algorithm~\ref{alg:rc} mention, we perform an bitwise XOR between original truth table $\textbf{M}$ and approximate truth table $\textbf{M}_{f_n}$, and obtain a corrector matrix $\textbf{R}$, which is then synthesized into the corrector circuit $Cir_c$. If we perform bitwise XOR between approximate truth table and corrector truth table, the original truth table is obtained. The corrector circuit is connected to rest sections with logic XOR for corresponding outputs. If 100\% accuracy is expected, besides all previous sections, the corrector circuit is also turned on.

%Algorithm~\ref{alg:rc} describes the procedure of generating runtime configurable approximate circuit, including computing a corrector circuit. $\text{QoR()}$ represents the Quality of Results metric. After obtaining the list of approximate sections $\textbf{Cir}$, corresponding outputs in each section are connected using logic OR, which are then connected to the corresponding output in corrector circuit $Cir_c$ with logic XOR. 

In Figure~\ref{fig:general_flow}, after factorizing input truth table for first two sections, a corrector truth table is computed to flip wrong bits. The corrector truth table is then synthesize into circuit $CONNECTOR$, which is connected to rest sections with bitwise XOR gate (gate $b$). If 100\% accuracy is needed, besides those sections discussed before, $CORRECTOR$ also has to be turned on.

==> tmp.tex <==
\begin{algorithm}[t!]
	\footnotesize
	\SetKwBlock{Begin}{begin}{end}
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	%\SetKwInOut{Phase1}{Phase 1}
	\Input{Accurate Circuit $ACir$, List of Objective Errors $\epsilon$ in ascending order}\label{alg:input}
	\Output{Runtime configurable circuit $Cir$ with self correcting capability}
	$subcircuits$ = Partition $ACir$ with hypergraph partitioning algorithm\\
	$f\_list$ = List of numbers of outputs for each of $subcircuits$ \\
	$design\_list$ = [$f\_list$] \\
	// Approximate all subcircuits \\
	\For{each subcircuit $s_i$ with $m_i$ outputs}
    {
     $\textbf{M}$ = Simulate subcircuit $s_i$ \\
        \For{ f = 1 to $m_i - 1$}
        {
        [$\textbf{B}_f$, $\textbf{C}_f$] = BMF($\textbf{M}$, f) \\
        $C_{s_i,f}$ = Synthesize $\textbf{B}_f$ and $\textbf{C}_f$
        }
    }	
    // Begin Design Space Exploration \\
    CurCir = ACir \\
    Let $f_i$ = $m_i$ for each $s_i$ in $subcircuits$ \\
    \While{$\epsilon$ is not empty}
    {
        \For{each subcircuit $s_i$ with $f_i > 1$}
        {
            $Cir'$ = $CurCir(s_i \rightarrow C_{s_i, f_i - 1})$ \\
            $loss_i$ = (power($Cir'$) - power($ACir$)) / QoR($Cir'$) \\
        }
        x = \arg\min_i\, loss_i \\
        $CurCir$ = $CurCir(s_x \rightarrow C_{s_x, f_x - 1})$ \\
        f_x = f_x - 1 \\
        \If{QoR($CurCir$) \geq \, $\epsilon$[0]}
        {
        $design\_list$.append($f\_list$ of best design so far) \\
        $\epsilon$.pop(0)
        }
    
    }	

	\Return $\textbf{Cir}$, $Cir_c$
	\caption{Runtime Configurable Approximate Circuit with Design Space Exploration}
		\label{alg:dse}
	%\vspace{-0.1in}
\end{algorithm}



\subsection{Accuracy Level v.s. Design Overhead}
\label{sec:acclevel_overhead}
As discussed in section~\ref{sec:capability}, in order to achieve self correcting capability, a corrector circuit is introduced. 


\subsection{Number of Accuracy Level}
\label{sec:number_accuracy}


\subsection{Runtime Configurable Accuracy}
\label{sec:result_1}
In this subsection, we evaluate the proposed methodology on 4-bit unsigned adder and 8-bit unsigned adder. Since the outputs of them represent numerical value, we use Mean Absolute Error as QoR metric here. Both circuits have limited number of inputs $m \leq 16$, which means BMF algorithm can be performed without partitioning. Therefore, we follow Algorithm~\ref{alg:rc} to evaluate both circuits, and obtain results in Table~\ref{table:adder}. Without circuit partitioning and design space exploration, the choice of accuracy level is actually limited by the number of primary outputs $m$, since we have at most $m-1$ factorization results. In practice, we first run BMF algorithm to assess all the possible accuracy level, and then choose the proper ones to synthesize. For both 4-bit unsigned adder and 8-bit unsigned adder, we choose 1 and 2 accuracy levels respectively with low MAE to evaluate, as well as full accuracy mode.

According to Table~\ref{table:adder}, 4-bit unsigned adder is evaluated at accuracy level 4.80\%, and 8-bit unsigned adder is evaluated at accuracy levels 1.50\% and 0.68\%. With these accuracy levels, power consumption is lower than original, which enables us to save power while choosing the proper accuracy level at runtime. 

However, the total area of runtime configurable circuit is larger than before, and more power are consumed than before if full accuracy level is chosen. On one hand, in order to achieve self correcting capability, we introduce corrector circuit, whose area and power depend on synthesis of a truth table. Also, the connecting OR/XOR gates between each accuracy level and corrector introduce overhead. On the other hand, according to Algorithm~\ref{alg:rc}, instead of directly synthesizing factorized truth table, we split it into groups of column-row pair and synthesize separately. We might lose some potential opportunities of logic optimization, and result in logic redundant.


\begin{table}
  %\footnotesize
  \centering
    \vspace{-0.1in}
    \caption{4-bit unsigned adder and 8-bit unsigned adder evaluated using the proposed methodology.}
  \begin{tabular}{||c|c|c|c|c|c||}
\hline
 & Accuracy & Approx. & Origin & Approx. & Origin \\
 & Level & Power & Power & Area & Area \\
 & MAE \%  & ($uW$) & ($uW$) &  ($um^2$) & ($um^2$) \\
 \hline
 4-bit & 4.80  &  31.20 & & & \\
 \cline{2-3}
 unsigned & Accurate  & 57.08 & 40.10 & 55.08 & 37.08 \\
 \cline{2-3}
 adder &-  & - & & & \\
 \hline
 8-bit & 1.50  &  31.90 & & & \\
 \cline{2-3}
 unsigned & 0.68  & 42.90 & 47.20 & 155.16 & 79.20 \\
 \cline{2-3}
 adder & Accurate  & 61.70 & & & \\
 \hline
  \end{tabular}
  %vspace*{-1mm}
  \vspace{0.1in}
  \label{table:adder}
\end{table}


\subsection{Partitioning and Design Space Exploration}
\label{sec:result_2}
In previous subsection, two small benchmarks are evaluated by factorizing truth table directly. As discussed in section~\ref{sec:DSE}, for larger input circuits, we first partition it into manageable subcircuits, and perform a design space exploration over these subcircuits. In this section, we choose 6 larger benchmarks from ISCAS and EPFL benchmark suite. 

For ISCAS, benchmark c1355, c1908 and c3540 are evaluated as general logic. We use normalized Hamming Distance as error metric. During design space exploration, we set objective error at 2\% and 4\%, and evaluate power consumption at two accuracy level as well as full accuracy mode. Table~\ref{table:ISCAS} demonstrates the results from three benchmarks. Similar to results in previous subsection, power consumption is reduced at each accuracy level compared to power of original circuit, except for  1.90\% accuracy level in c1355. Design area and power of full accuracy mode are increased due to overhead of corrector circuit and logic redundance. 

\begin{table}
  %\footnotesize
  \centering
    \vspace{-0.1in}
    \caption{3 benchmarks from ISCAS evaluated using circuit partitioning and DSE.}
  \begin{tabular}{||c|c|c|c|c|c||}
\hline
 & Accuracy & Approx. & Origin & Approx. & Origin \\
 & Level & Power & Power & Area & Area \\
 & HD \%  & ($uW$) & ($uW$) &  ($um^2$) & ($um^2$) \\
 \hline
  & 3.97  &  102.00 & & & \\
 \cline{2-3}
 c1355 & 1.90  & 131.73 & 124.00 & 779.04 & 629.28 \\
 \cline{2-3}
  & Accurate  & 149.01 & & & \\
 \hline
  & 3.97  &  24.00 & & & \\
 \cline{2-3}
 c1908 & 1.58  & 64.72 & 70.10 & 458.44 & 388.80 \\
 \cline{2-3}
  & Accurate  & 83.08 & & & \\
 \hline
   & 3.49  &  35.10 & & & \\
 \cline{2-3}
 c432 & 1.50  & 41.05 & 42.00 & 200.52 & 167.04 \\
 \cline{2-3}
  & Accurate  & 43.56 & & & \\
 \hline
  \end{tabular}
  %vspace*{-1mm}
  \vspace{0.1in}
  \label{table:ISCAS}
\end{table}

For EPFL, benchmark adder, barrel shifter and max are evaluated. Since EPFL benchmark suite  does not provide bit numbering of outputs, we  use normalized Hamming distance as QoR metric. For each of three benchmark, objective errors are set to 1\% and 2\%. Table~\ref{table:EPFL} demonstrates the results from three benchmarks. The results show similar trend with previous sets of experiments. It proves that our methodology is able to generate runtime configurable approximate accuracy that saves power utilization by applying an accuracy level at run time. 



\begin{table}
  %\footnotesize
  \centering
    \vspace{-0.1in}
    \caption{3 benchmarks from EPFL evaluated using circuit partitioning and DSE.}
  \begin{tabular}{||c|c|c|c|c|c||}
\hline
 & Accuracy & Approx. & Origin & Approx. & Origin \\
 & Level & Power & Power & Area & Area \\
 & HD \%  & ($uW$) & ($uW$) &  ($um^2$) & ($um^2$) \\
 \hline
  & 1.95  &  74.20 & & & \\
 \cline{2-3}
 Adder & 0.97  & 83.36 & 84.40 & 2541.96 & 1966.68 \\
 \cline{2-3}
  & Accurate  & 94.45 & & & \\
 \hline
 & 1.93  &  715.00 & & & \\
 \cline{2-3}
 Bar  & 0.96 & 748.09 & 767.00 & 3789.72 & 3412.80 \\
 \cline{2-3}
   & Accurate  & 750.29 & & & \\
 \hline
   & 1.99 &  327.09 & & & \\
 \cline{2-3}
 Max & 0.97  & 369.00 & 372.00 & 3653.20 & 3250.80 \\
 \cline{2-3}
  & Accurate  & 427.20 & & & \\
 \hline
  \end{tabular}
  %vspace*{-1mm}
  \vspace{0.1in}
  \label{table:EPFL}
\end{table}



\newpage


\subsection{Number of Accuracy Levels}
\label{sec:num_level}
In this subsection, we evaluate proposed methodology on 8-bit adder with different number of accuracy levels, to analyse the relationship between number of accuracy levels and power consumption/area saving. Based on the conclusion of subsection~\ref{sec:obj_error}, we choose error thresholds from 1\% to 6\%. We start with 2-level runtime configurable approximate design, where error thresholds are full accuracy and 6\%. Error thresholds between 1\% and 6\% are added to form 3-level, 4-level and 5-level design. For each runtime approximate design, we evaluate {\it relative power} under each accuracy level, and {\it relative area} as well. Figure~\ref{fig:num_level} compares 4 designs with different number of accuracy levels. One one hand, the relative area becomes smaller with more accuracy levels. On the other hand, with more accuracy levels, the factorized truth tables are splitted into more groups of matrices, each of which is synthesized {\it individually}. In this case, we lose opportunity to optimize logic synthesis across different blocks, where power consumption under lower error thresholds (or full accuracy) becomes higher. As Figure~\ref{fig:num_level} shows, with 3-level design, we are able to save power by running under each approximate mode. However, with 4-level design, power consumption under 2\% error threshold already exceeds power of original circuit, where power is {\it not} saved by trading off accuracy. Based on Figure~\ref{fig:num_level}, we conclude that 3-level approximate design is a good choice.
% In this subsection, we analyse the trade-off between design overhead and number of accuracy levels. We evaluate our methodology on 8-bit adder with 2-5 accuracy levels and summarize results in Table~\ref{table:num_level}. With more accuracy levels, we may observe that runtime configurable design saves more chip area compared to baseline, since blocks are re-used for more accuracy levels. However, the power consumption in full accurate mode increases dramatically. When having more accuracy levels, the truth table of input circuit is splitted into more groups of matrices, which are synthesized {\it individually}. In this process, we lose opportunity to optimize logic synthesis across different blocks, which leads to higher power consumption than the baseline. Based on Table~\ref{table:num_level}, 3 accuracy levels might be a descent choice, since power is saved in all approximate levels, and power consumption in full accurate mode is not too high.

\begin{figure}[h]
	\begin{center}
	
    \includegraphics[width=0.5\textwidth]{figures/num_levels.png}
		%\includegraphics[width=0.45\textwidth]{figures/circuit_level.png}
		%\vspace{-0.1in}
		\caption{Runtime configurable design of 8-bit adder with different number of accuracy levels.}
		\label{fig:num_level}
	\end{center}
\end{figure}

 
\subsection{Runtime configurable design}
\label{sec:final}

\begin{table}[h!]
  %\footnotesize
  \centering
    \vspace{-0.1in}
    \caption{7 benchmarks from BACS evaluated using circuit partitioning and DSE.}
  \begin{tabular}{||c|c|c|c|c|c||}
\hline
 & Accuracy & Approx. & Baseline & Approx. & Baseline \\
 & Level & Power & Power & Area & Area \\
 & \%  & ($uW$) & ($uW$) &  ($um^2$) & ($um^2$) \\
 \hline
  & Accurate  & 79.87   & & & \\
 \cline{2-3}
 x2 & 7.03  & 36.03 & 67.40 & 93.24 & 101.16 \\
 \cline{2-3}
  & 11.27  & 29.28 & & & \\
 \hline
 & Accurate  &  87.01 & & & \\
 \cline{2-3}
 mac  & 1.86 & 69.46 & 85.32 & 222.48 & 416.52 \\
 \cline{2-3}
   & 3.04  & 64.01 & & & \\
 \hline
   & Accurate &  138.32 & & & \\
 \cline{2-3}
 buttfly & 0.10 & 74.09 & 101.51 & 542.16 & 811.44 \\
 \cline{2-3}
  & 0.33  & 68.92 & & & \\
 \hline
 
    & Accurate &   & & & \\
 \cline{2-3}
 abs\_diff &  &  &  &  & \\
 \cline{2-3}
  &   &  & & & \\
 \hline
 
     & Accurate &   & & & \\
 \cline{2-3}
 mult16 &  &  &  &  & \\
 \cline{2-3}
  &   &  & & & \\
 \hline
 
      & Accurate & 270.72   & & & \\
 \cline{2-3}
 mult8 & 0.18 & 238.76  & 220.66 & 934.2 & 1559.16 \\
 \cline{2-3}
  &  0.81 & 142.65 & & & \\
 \hline

     & Accurate & 139.47  & & & \\
 \cline{2-3}
 adder32 & 0.01 & 80.99  & 111.54 & 549.72  &  754.56 \\
 \cline{2-3}
  & 0.42  & 52.94  & & & \\
 \hline
  \end{tabular}
  %vspace*{-1mm}
  \vspace{0.1in}
  \label{table:BACS}
\end{table}

Based on subsection~\ref{sec:obj_error} and~\ref{sec:num_level}, we evaluate our methodology on BACS benchmark, where a runtime configurable design with 3 accuracy levels is created for each benchmark. All benchmarks are evaluated using circuit partitioning and DSE. We summarize results in Table~\ref{table:BACS}. Compared to baseline circuit, our runtime configurable design saves XX\% chip area on average. When running in approximate levels, the runtime configurable design also has significant saving in terms of power consumption. Although our methodology makes compromises on power consumption of full accurate mode,  the design overhead is controlled within reasonable amount by design space exploration and approach discussed in subsection~\ref{sec:overhead},

